The Cost of Local and Global Fairness in Federated Learning

With the emerging application of Federated Learning (FL) in finance, hiring and healthcare, FL models are regulated to be fair, preventing disparities with respect to legally protected attributes such as race or gender. Two concepts of fairness are important in FL: global and local fairness. Global fairness addresses the disparity across the entire population and local fairness is concerned with the disparity within each client. Prior fair FL frameworks have improved either global or local fairness without considering both. Furthermore, while the majority of studies on fair FL focuses on binary settings, many real-world applications are multi-class problems. This paper proposes a framework that investigates the minimum accuracy lost for enforcing a specified level of global and local fairness in multi-class FL settings. Our framework leads to a simple post-processing algorithm that derives fair outcome predictors from the Bayesian optimal score functions. Experimental results show that our algorithm outperforms the current state of the art (SOTA) with regard to the accuracy-fairness tradoffs, computational and communication costs. Codes are available at: https://github.com/papersubmission678/The-cost-of-local-and-global-fairness-in-FL .

==> 0_re_abstract.tex <==
\begin{abstract}

 Federated Learning (FL) is a distributed machine learning framework in which a set of local clients collaboratively learn a shared global model while retaining all  data locally. With the emerging application of FL in finance, hiring and medical diagnosis, those models are regulated to be group fair.  Group fairness requires that models do not exhibit disparities between groups based on legally protected attributes. There are two concepts of group fairness in FL: global fairness and local fairness. Global fairness addresses the overall disparity across all population, while local fairness addresses the disparity within each client. Existing literature has proposed FL frameworks to improve either global or local fairness. However, the minimum accuracy costs for improving both fairness concepts remain unexplored. This paper provides a framework that investigates the maximum achievable accuracy under a specified level of local and global fairness in multi-class setting. Our framework can be implemented in FL by solving a linear program with polynomial computational complexity.  Experimental results show that our implementation outperforms the current state of the art (SOTA) in terms of the accuracy cost for fairness, communication efficiency and computational cost. 
 \end{abstract}
